Magnification, dust and time-delay constraints from the first resolved strongly lensed Type Ia supernova

We report lensing magnifications, extinction, and time-delay estimates for the first resolved, multiply-imaged Type Ia supernova iPTF16geu, at $z = 0.409$, using $Hubble\,Space\,Telescope$ ($HST$) observations in combination with supporting ground-based data. Multi-band photometry of the resolved images provides unique information about the differential dimming due to dust in the lensing galaxy. Using $HST$ and Keck AO reference images taken after the SN faded, we obtain a total lensing magnification for iPTF16geu of $\mu = 67.8^{+2.6}_{-2.9}$, accounting for extinction in the host and lensing galaxy. As expected from the symmetry of the system, we measure very short time-delays for the three fainter images with respect to the brightest one: -0.23 $\pm$ 0.99, -1.43 $\pm$ 0.74 and 1.36 $\pm$ 1.07 days. Interestingly, we find large differences between the magnifications of the four supernova images, even after accounting for uncertainties in the extinction corrections: $\Delta m_1 = -3.88^{+0.07}_{-0.06}$, $\Delta m_2 = -2.99^{+0.09}_{-0.08}$, $\Delta m_3 = -2.19^{+0.14}_{-0.15}$ and $\Delta m_4 = -2.40^{+0.14}_{-0.12}$ mag, discrepant with model predictions suggesting similar image brightnesses. A possible explanation for the large differences is gravitational lensing by substructures, micro- or millilensing, in addition to the large scale lens causing the image separations. We find that the inferred magnification is insensitive to the assumptions about the dust properties in the host and lens galaxy.

==> ground_photometry_16geu.tex <==
\begin{table}
\begin{tabular}{cccc}
time & band & flux & fluxerr \\
57636.335 & P48R & 52.481 & 9.6673 \\
57637.181 & P48R & 80.91 & 12.668 \\
57637.329 & P48R & 83.946 & 11.598 \\
57638.177 & P48R & 98.175 & 10.851 \\
57638.328 & P48R & 86.298 & 11.128 \\
57639.227 & P48R & 114.82 & 13.747 \\
57639.337 & P48R & 109.65 & 10.099 \\
57640.215 & P48R & 130.62 & 13.233 \\
57640.324 & P48R & 130.62 & 13.233 \\
57641.201 & P48R & 165.96 & 18.342 \\
57641.318 & P48R & 152.76 & 12.662 \\
57642.196 & P48R & 205.12 & 18.892 \\
57642.31 & P48R & 177.01 & 17.934 \\
57646.329 & P60r & 220.8 & 16.269 \\
57646.331 & P60i & 277.97 & 10.241 \\
57646.333 & P60g & 106.66 & 12.771 \\
57648.359 & P60r & 270.4 & 37.357 \\
57648.361 & P60i & 325.09 & 17.965 \\
57648.364 & P60g & 111.69 & 16.459 \\
57654.14 & P48R & 288.4 & 18.594 \\
57655.115 & P48R & 283.14 & 23.47 \\
57655.24 & P48R & 283.14 & 18.255 \\
57656.124 & P48R & 310.46 & 22.875 \\
57656.25 & P48R & 277.97 & 20.482 \\
57657.148 & P48R & 272.9 & 17.594 \\
57657.246 & P48R & 270.4 & 24.904 \\
57658.132 & P48R & 280.54 & 20.671 \\
57658.175 & P48R & 272.9 & 17.594 \\
57659.245 & P48R & 285.76 & 23.687 \\
57660.149 & P48R & 251.19 & 20.822 \\
57661.109 & P48R & 246.6 & 20.442 \\
57661.154 & P48R & 231.21 & 19.165 \\
57662.104 & P48R & 265.46 & 26.895 \\
57662.228 & P48R & 237.68 & 17.513 \\
57663.119 & P48R & 226.99 & 16.725 \\
57663.222 & P48R & 224.91 & 18.643 \\
57664.17 & P48R & 229.09 & 18.99 \\
57664.249 & P60r & 222.84 & 18.472 \\
57664.251 & P60i & 346.74 & 28.742 \\
57664.261 & P60r & 235.5 & 13.014 \\
57664.263 & P60i & 316.23 & 55.339 \\
57664.264 & P60g & 48.306 & 8.0084 \\
57665.294 & P60r & 205.12 & 18.892 \\
57665.296 & P60i & 319.15 & 91.125 \\
57665.298 & P60g & 52.966 & 7.8054 \\
57667.106 & P60r & 192.31 & 37.196 \\
57668.099 & P48R & 203.24 & 18.719 \\
57668.216 & P48R & 190.55 & 17.55 \\
57669.113 & P48R & 180.3 & 23.249 \\
57669.146 & P60r & 144.54 & 26.626 \\
57670.098 & P48R & 194.09 & 25.027 \\
57670.124 & J-SPM & 482.61409327 & 33.45520316 \\
57670.124 & Y-SPM & 277.2043237577699 & 33.983922850388296 \\
57670.124 & i-SPM & 252.34807724805728 & 5.516908278323143 \\
57670.124 & r-SPM & 135.89391171008 & 5.637233096411137 \\
57670.124 & z-SPM & 252.81334798341183 & 11.378475011996443 \\
57670.171 & P60r & 162.93 & 6.0025 \\
57670.173 & P60i & 251.19 & 11.568 \\
57670.174 & P60g & 25.351 & 4.2029 \\
57670.225 & P60r & 145.88 & 12.093 \\
57670.226 & P60i & 244.34 & 51.761 \\
57671.157 & Y-SPM & 261.57726827191084 & 30.79629530207029 \\
57671.157 & J-SPM & 489.327924086 & 35.17721145 \\
57671.157 & i-SPM & 249.11506965638617 & 5.446227310427986 \\
57671.157 & r-SPM & 130.25667861366887 & 5.633162565017329 \\
57671.157 & z-SPM & 228.03420720004186 & 11.463357729034698 \\
57671.225 & P60i & 226.99 & 367.95 \\
57671.235 & P60r & 125.89 & 12.755 \\
57671.237 & P60i & 242.1 & 187.31 \\
57673.188 & P60r & 120.23 & 135.09 \\
57673.189 & P60i & 222.84 & 28.735 \\
57673.211 & P60r & 118.03 & 13.045 \\
57673.213 & P60i & 255.86 & 141.39 \\
57674.123 & P60r & 131.83 & 18.212 \\
57674.125 & P60i & 203.24 & 11.231 \\
57674.208 & P60r & 96.383 & 12.428 \\
57674.21 & P60i & 237.68 & 78.809 \\
57675.155 & r-SPM & 85.90135215053965 & 4.9172074179607534 \\
57675.155 & J-SPM & 512.38923866 & 35.07982474 \\
57675.155 & Y-SPM & 274.1574171927881 & 33.166874324129054 \\
57675.155 & z-SPM & 212.81390459827134 & 11.81207988690204 \\
57675.155 & i-SPM & 210.66869257394166 & 4.984933911152638 \\
57680.204 & P60r & 61.944 & 89.573 \\
57681.102 & P48R & 88.716 & 14.708 \\
57682.096 & P48R & 81.658 & 11.282 \\
57682.139 & P48R & 94.624 & 12.201 \\
57682.23 & P60r & 64.863 & 12.546 \\
57682.231 & P60i & 145.88 & 29.56 \\
57683.093 & P48R & 85.507 & 11.026 \\
57683.113 & r-SPM & 50.07258356403346 & 4.4058445990804245 \\
57683.113 & z-SPM & 204.36193210844672 & 12.052759217430776 \\
57683.113 & i-SPM & 155.02437888710415 & 4.779388587212708 \\
57683.113 & Y-SPM & 330.8262788556975 & 41.09192008556482 \\
57683.113 & J-SPM & 562.34132519 & 34.62564343 \\
57683.138 & P48R & 90.365 & 9.1552 \\
57684.151 & J-SPM & 530.15150668 & 34.01635309 \\
57684.151 & Y-SPM & 299.2264636608192 & 35.22885072533779 \\
57684.151 & z-SPM & 207.01413487910415 & 11.490167917015697 \\
57684.151 & i-SPM & 153.88631498199555 & 4.744302172555592 \\
57684.151 & r-SPM & 37.84425847170936 & 4.208594896873137 \\
57685.116 & i-SPM & 153.88631498199555 & 4.744302172555592 \\
57685.116 & J-SPM & 575.97018125 & 34.96677439 \\
57685.116 & r-SPM & 39.12010393873516 & 4.5420935855045315 \\
57685.116 & Y-SPM & 313.0401190096241 & 31.720513329627806 \\
57685.116 & z-SPM & 182.9784734295412 & 11.740531305048364 \\
57687.117 & Y-SPM & 320.62693245054675 & 37.226831899637205 \\
57687.117 & J-SPM & 521.915265835 & 34.31519574 \\
57687.117 & i-SPM & 131.58306550959165 & 4.992890579567515 \\
57687.117 & z-SPM & 196.06496672266033 & 11.563424804712383 \\
57687.117 & r-SPM & 35.35086133619967 & 4.219364681729516 \\
57687.13 & P60r & 39.811 & 31.534 \\
57687.132 & P60i & 129.42 & 10.728 \\
57688.112 & r-SPM & 35.74374062644806 & 4.324187780037377 \\
57688.112 & Y-SPM & 312.751931140798 & 44.34112278627515 \\
57688.112 & z-SPM & 185.35316234148144 & 12.53077504650463 \\
57688.112 & i-SPM & 133.1680376269981 & 4.816817943048221 \\
57688.113 & P60r & 40.551 & 34.361 \\
57688.114 & J-SPM & 548.02453218 & 35.16314819 \\
57688.115 & P60i & 120.23 & 25.469 \\
57690.114 & J-SPM & 520.47515117 & 34.29189271 \\
57690.114 & z-SPM & 155.8834467704389 & 11.605484457491144 \\
57690.114 & r-SPM & 26.91534803926914 & 4.0277614686454974 \\
57690.114 & i-SPM & 132.8005886243731 & 4.803526953855027 \\
57690.114 & Y-SPM & 367.790070422387 & 48.63628491231049 \\
57691.112 & z-SPM & 168.73298906258066 & 11.696708629225014 \\
57691.112 & i-SPM & 121.89895989248662 & 4.62542931454891 \\
57691.112 & r-SPM & 22.719564377352643 & 3.9263962093199787 \\
57691.112 & J-SPM & 546.00924975 & 34.56299816 \\
57691.112 & Y-SPM & 301.4393884279469 & 34.01562271904743 \\
57692.14 & J-SPM & 487.07966649 & 33.76476035 \\
57692.14 & r-SPM & 30.283076942657782 & 4.14943118076755 \\
57692.14 & z-SPM & 145.8814260275349 & 11.357355512671745 \\
57692.14 & i-SPM & 123.25370982033455 & 4.676835003618706 \\
57692.14 & Y-SPM & 330.5217168699794 & 42.11856655731913 \\
57693.15 & J-SPM & 537.52664879 & 41.3914952 \\
57693.15 & r-SPM & 23.85613039930911 & 4.801523219676646 \\
57693.15 & z-SPM & 117.48975549395303 & 12.873300391752224 \\
57693.15 & i-SPM & 125.7766432451253 & 5.439416126856699 \\
57695.108 & P60i & 84.723 & 138.12 \\
57695.18 & P60i & 91.201 & 21.84 \\
57696.08 & P60i & 103.75 & 18.156 \\
57696.082 & P60i & 148.59 & 15.055 \\
57697.105 & P60r & 30.2 & 54.239 \\
57697.107 & P60i & 66.069 & 12.779 \\
57697.109 & P60i & 85.507 & 6.3004 \\
57700.096 & P60i & 114.82 & 106.81 \\
57702.148 & P60i & 92.045 & 22.042 \\
57702.15 & P60i & 83.176 & 16.088 \\
57705.163 & P60i & 80.168 & 16.244 \\
57723.104 & r-SPM & 9.718517029401701 & 0.7731121916130004 \\
57723.104 & Y-SPM & 132.06872951464237 & 25.996914551110905 \\
57723.104 & i-SPM & 48.261409326852096 & 4.489045533375602 \\
57723.104 & z-SPM & 67.48387308707574 & 11.353232319555524 \\
57723.104 & Y-SPM & 113.76272858 & 31.42478806 \\
\end{tabular}
\end{table}


==> host1_model.tex <==
\begin{tabular}{l | r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l}
\hline\hline
Filter & \multicolumn{2}{c}{$a_0$} & \multicolumn{2}{c}{$a_1$} & \multicolumn{2}{c}{$b_1$} & \multicolumn{2}{c}{$a_2$} & \multicolumn{2}{c}{$b_2$}\\
  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{}\\
\hline
$K_s$ & 1.47E$+$00 & (1E$-$02) & $-$2.97E$-$01 & (3E$-$03) & 2.56E$-$01 & (3E$-$03) & $-$1.41E$-$01 & (2E$-$03) & 3.53E$-$02 & (2E$-$03)\\
$H$ & 5.16E$-$01 & (3E$-$03) & $-$1.07E$-$01 & (2E$-$03) & 8.64E$-$02 & (2E$-$03) & $-$4.76E$-$02 & (1E$-$03) & 1.75E$-$03 & (2E$-$03)\\
$F160W$ & 1.01E$+$02 & (1E$+$00) & $-$1.48E$+$01 & (7E$-$01) & 2.33E$+$01 & (7E$-$01) & $-$2.39E$+$01 & (6E$-$01) & 4.88E$+$00 & (6E$-$01)\\
$J$ & 2.78E$-$01 & (5E$-$03) & $-$6.93E$-$02 & (2E$-$03) & 4.75E$-$02 & (2E$-$03) & $-$3.43E$-$02 & (1E$-$03) & $-$1.52E$-$02 & (1E$-$03)\\
$F110W$ & 1.40E$+$02 & (2E$+$00) & $-$2.28E$+$01 & (1E$+$00) & 2.62E$+$01 & (1E$+$00) & $-$3.85E$+$01 & (1E$+$00) & $-$2.03E$+$00 & (1E$+$00)\\
$F814W$ & 1.41E$+$00 & (3E$-$02) & $-$1.11E$-$01 & (8E$-$03) & 1.15E$-$01 & (8E$-$03) & $-$1.51E$-$01 & (9E$-$03) & $-$8.07E$-$02 & (9E$-$03)\\
$F625W$ & 8.06E$-$01 & (4E$-$02) & 4.52E$-$02 & (7E$-$03) & 2.73E$-$02 & (7E$-$03) & $-$9.13E$-$02 & (9E$-$03) & $-$4.77E$-$02 & (8E$-$03)\\
$F475W$ & 1.07E$-$01 & (2E$-$02) & $^*$0.00E$+$00 &  & $^*$0.00E$+$00 &  & $^*$0.00E$+$00 &  & $^*$0.00E$+$00 & \\
\hline
\end{tabular}


==> host2_model.tex <==
\begin{tabular}{l | r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l}
\hline\hline
Filter & \multicolumn{2}{c}{$a_3$} & \multicolumn{2}{c}{$b_3$} & \multicolumn{2}{c}{$c_0$} & \multicolumn{2}{c}{$c_1$} & \multicolumn{2}{c}{$d_1$}\\
  & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{$('')$} & \multicolumn{2}{c}{$('')$} & \multicolumn{2}{c}{$('')$}\\
\hline
$K_s$ & 1.76E$-$01 & (2E$-$03) & $-$1.63E$-$01 & (3E$-$03) & 5.831E$-$01 & (3E$-$04) & 3.08E$-$02 & (3E$-$04) & $-$3.54E$-$02 & (3E$-$04)\\
$H$ & 5.72E$-$02 & (2E$-$03) & $-$4.73E$-$02 & (2E$-$03) & 5.787E$-$01 & (8E$-$04) & 3.38E$-$02 & (8E$-$04) & $-$3.11E$-$02 & (8E$-$04)\\
$F160W$ & $-$1.15E$+$00 & (8E$-$01) & $-$1.26E$+$01 & (6E$-$01) & $^*$5.787E$-$01 &  & $^*$3.38E$-$02 &  & $^*$$-$3.11E$-$02 & \\
$J$ & 3.46E$-$02 & (1E$-$03) & $-$2.00E$-$02 & (1E$-$03) & 5.911E$-$01 & (1E$-$03) & 4.49E$-$02 & (1E$-$03) & $-$1.69E$-$02 & (9E$-$04)\\
$F110W$ & $-$4.29E$-$01 & (2E$+$00) & $-$1.54E$+$01 & (1E$+$00) & $^*$5.911E$-$01 &  & $^*$4.49E$-$02 &  & $^*$$-$1.69E$-$02 & \\
$F814W$ & 9.74E$-$02 & (9E$-$03) & $-$1.71E$-$01 & (9E$-$03) & 5.784E$-$01 & (1E$-$03) & 3.51E$-$02 & (8E$-$04) & $-$6.58E$-$03 & (8E$-$04)\\
$F625W$ & 1.74E$-$02 & (9E$-$03) & $-$1.13E$-$01 & (9E$-$03) & 5.788E$-$01 & (2E$-$03) & 3.28E$-$02 & (1E$-$03) & 5.30E$-$03 & (1E$-$03)\\
$F475W$ & $^*$0.00E$+$00 &  & $^*$0.00E$+$00 &  & $^*$5.788E$-$01 &  & $^*$3.28E$-$02 &  & $^*$5.30E$-$03 & \\
\hline\hline
\end{tabular}


==> parameters_tab.tex <==
 \begin{table*}
\centering
\caption{This table summarises the resulting best fit parameters by fitting an \texttt{sncosmo} model to the ground-based and HST observations. For each image, we present the time of maximum, t$_{max}$ (relative to image 1), host galaxy colour excess (which is treated as being the same for each image), the lens galaxy colour excess as well as the magnification for each image (given as the 68$\%$ credible region of the posterior distribution). Our fiducial case assumes $R_V =2$ in both the host and the lens galaxy. We also present the parameters values assuming host $R_V =2$ and lens $R_V$ as a free parameter (for two cases, one assuming a single $R_V$ for the lens galaxy and the other assuming different $R_V$'s for each image) as well as the case with host and lens $R_V$ fixed to the Milky Way value of 3.1.}
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|}
\hline
Parameter & Image 1 & Image 2 &  Image 3 & Image 4 \\
\hline\hline
&& Fiducial Fit Parameters \\
 {\bf t$_{\rm max}$} & {\bf 57652.80 ($\pm$ 0.33)} & {\bf -0.23 ($\pm$  0.99)} & {\bf -1.43  ($\pm$ 0.74)} & {\bf 1.36 ($\pm$ 1.07)} \\
 {\bf stretch ($s$)} & {\bf 0.99 ($\pm$ 0.01)} & {\bf Same as Image 1}  & {\bf Same as Image 1}  & {\bf Same as Image 1}  \\
 {\bf E(B-V)|$_{\rm host}$}   &  {\bf 0.29 ($\pm$ 0.05)} &   {\bf Same as Image 1} & {\bf Same as Image 1} & {\bf Same as Image 1}  \\
 {\bf E(B-V)|$_{\rm lens}$}  &  {\bf 0.06 ($\pm$ 0.08)} &  {\bf 0.17 ($\pm$ 0.08)} & {\bf 0.42 ($\pm$ 0.09)} & {\bf 0.94 ($\pm$ 0.07)} \\
 {\bf Magnification} & {\bf $-3.88^{+0.07}_{-0.06}$} & {\bf $-2.99^{+0.09}_{-0.08}$} & {\bf $-2.19^{+0.14}_{-0.15}$} & {\bf $-2.40^{+0.14}_{-0.12}$ }
\\
 \\
 && Fit with Reddening Assumptions Modified && \\
 
t$_{\rm max}$ (free lens $R_V$, host $R_V$ = 2) &  57652.9 ($\pm$ 0.20) & -0.31 ($\pm$  0.93) & -1.84  ($\pm$ 0.90) & 0.77 ($\pm$ 1.27) \\
t$_{\rm max}$ (fixed lens, host $R_V = 3.1$) &  57652.7 ($\pm$ 0.38) & 0.11 ($\pm$  0.91) & -0.85  ($\pm$ 1.08) & -0.41 ($\pm$ 2.27) \\

stretch ($s$; free lens $R_V$, host $R_V$ = 2) & 1.00 ($\pm$ 0.01) & Same as Image 1 & Same as Image 1 & Same as Image 1 & Same as Image 1 \\
stretch (s; fixed lens, host $R_V = 3.1$) & 1.01 ($\pm$ 0.01) & Same as Image 1 & Same as Image 1 & Same as Image 1 & Same as Image 1 \\
E(B-V)|$_{\rm host}$  (free lens $R_V$, host $R_V$ = 2) & 0.18 ($\pm$ 0.05) & Same as Image 1 & Same as Image 1 & Same as Image 1  \\
E(B-V)|$_{\rm host}$  (fixed lens, host $R_V = 3.1$)& 0.17 ($\pm$ 0.08) & Same as Image 1 & Same as Image 1 & Same as Image 1  \\


E(B-V)|$_{\rm lens}$(free lens $R_V$, host $R_V$=2)  &  0.26 ($\pm$ 0.09) &  0.41 ($\pm$ 0.10) & 0.78 ($\pm$ 0.12) & 1.58 ($\pm$ 0.14) \\
E(B-V)|$_{\rm lens}$ (fixed lens, host $R_V = 3.1$)  &  0.13 ($\pm$ 0.08) &  0.20 ($\pm$ 0.09) & 0.40 ($\pm$ 0.09) & 0.70 ($\pm$ 0.09) \\
R|$_{\rm V,lens}$ (free lens $R_V$) & $< 1.8$ & Same as Image 1 & Same Image 1 & Same as Image 1 \\

Magnification (free lens $R_V$) & {\bf $-3.78^{+0.09}_{-0.10}$} & {\bf $-2.85^{+0.10}_{-0.11}$} & {\bf $-1.86^{+0.15}_{-0.15}$} & {\bf $-1.98^{+0.16}_{-0.17}$ }\\
Magnification (fixed lens, host $R_V = 3.1$) & 
{\bf $-4.04^{+0.12}_{-0.08}$} & {\bf $-3.18^{+ 0.14}_{-0.13}$} & {\bf $-2.39^{+0.22}_{-0.23}$} & {\bf $-2.57^{+0.11}_{-0.07}$ }
\\

\hline
\end{tabular}}
\label{tab:params}
\end{table*}

==> parameters_tab_rahmanphotometry.tex <==
 \begin{table*}
\centering
\caption{This table summarises the resulting best fit parameters by fitting an \texttt{sncosmo} model to the ground-based and HST observations. For each image, we present the time of maximum, t$_{max}$ (relative to image 1), host galaxy colour excess (which is treated as being the same for each image), the lens galaxy colour excess as well as the magnification for each image (given as the 68$\%$ credible region of the posterior distribution). Our fiducial case assumes $R_V =2$ in both the host and the lens galaxy. We also present the parameters values assuming host $R_V =2$ and lens $R_V$ as a free parameters as well as the case with host and lens $R_V$ fixed to the Milky Way value of 3.1.}
\resizebox{\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|}
\hline
Parameter & Image 1 & Image 2 &  Image 3 & Image 4 \\
\hline\hline
&& Fiducial Fit Parameters &\\
 {\bf t$_{max}$} & {\bf 57653.46 ($\pm$ 0.35)} & {\bf -0.39 ($\pm$  0.63)} & {\bf -1.49  ($\pm$ 0.74)} & {\bf 1.32 ($\pm$ 0.77)} \\
 {\bf E(B-V)|$_{\rm host}$}   &  {\bf 0.23 ($\pm$ 0.06)} &   {\bf Same as Image 1} & {\bf Same as Image 1} & {\bf Same as Image 1}  \\
 {\bf E(B-V)|$_{\rm lens}$}  &  {\bf 0.12 ($\pm$ 0.08)} &  {\bf 0.24 ($\pm$ 0.08)} & {\bf 0.49 ($\pm$ 0.09)} & {\bf 1.02 ($\pm$ 0.10)} \\
 {\bf Magnification} & {\bf $-3.88^{+0.11}_{-0.09}$} & {\bf $-2.99^{+0.14}_{-0.15}$} & {\bf $-2.12^{+0.16}_{-0.12}$} & {\bf $-2.40^{+0.12}_{-0.14}$ }
\\
 \\
 && Fit with Reddening Assumptions Modified && \\
 
t$_{max}$ (free lens $R_V$, host $R_V$ = 2) &  57653.45 ($\pm$ 0.35) & -0.933 ($\pm$  0.887) & -2.678  ($\pm$ 1.534) & -0.347 ($\pm$ 2.157) \\
t$_{max}$ (fixed lens, host $R_V = 3.1$) &  57653.25 ($\pm$ 0.35) & -0.99 ($\pm$  0.91) & -2.55  ($\pm$ 1.52) & -0.41 ($\pm$ 2.27) \\



E(B-V)|$_{\rm host}$  (free lens $R_V$, host $R_V$ = 2) & 0.322 ($\pm$ 0.018) & Same as Image 1 & Same as Image 1 & Same as Image 1  \\
E(B-V)|$_{\rm host}$  (fixed lens, host $R_V = 3.1$)& 0.04 ($\pm$ 0.05) & Same as Image 1 & Same as Image 1 & Same as Image 1  \\


E(B-V)|$_{\rm lens}$(free lens $R_V$, host $R_V$=2)  &  0.189 ($\pm$ 0.010) &  0.074 ($\pm$ 0.104) & 0.578 ($\pm$ 0.296) & 1.522 ($\pm$ 0.504) \\
E(B-V)|$_{\rm lens}$ (fixed lens, host $R_V = 3.1$)  &  0.22 ($\pm$ 0.06) &  0.20 ($\pm$ 0.07) & 0.26 ($\pm$ 0.11) & 0.60 ($\pm$ 0.18) \\


Magnification (free lens $R_V$) & {\bf $-3.940^{+0.095}_{-0.088}$} & {\bf $-2.817^{+0.256}_{-0.189}$} & {\bf $-2.229^{+0.779}_{-0.333}$} & {\bf $-2.095^{+1.806}_{-0.452}$ }\\
Magnification (fixed lens, host $R_V = 3.1$) & 
{\bf $-4.01^{+0.12}_{-0.08}$} & {\bf $-2.93^{+ 0.25}_{-0.19}$} & {\bf $-2.32^{+0.76}_{-0.32}$} & {\bf $-2.12^{+1.47}_{-0.40}$ }
\\

\hline
\end{tabular}}
\label{tab:params}
\end{table*}

==> resolved_photometry.tex <==
\begin{tabular}{r c r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r @{\hspace{0.5em}} l r}
\hline\hline
\multicolumn{1}{c}{MJD} & \multicolumn{1}{c}{Filter} & \multicolumn{2}{c}{Flux \#1} & \multicolumn{2}{c}{Flux \#2} & \multicolumn{2}{c}{Flux \#3} & \multicolumn{2}{c}{Flux \#4} & \multicolumn{1}{c}{ZP}\\
\multicolumn{1}{c}{(days)} & & \multicolumn{2}{c}{(counts/s)} & \multicolumn{2}{c}{(counts/s)} & \multicolumn{2}{c}{(counts/s)} & \multicolumn{2}{c}{(counts/s)} & \multicolumn{1}{c}{(mag)}\\
\hline
57681.64 & $F110W$ & 5.17E$+$02 & (1E$+$01,1E$+$01) & 1.74E$+$02 & (8E$+$00,1E$+$01) & 1.02E$+$02 & (8E$+$00,2E$+$01) & 4.98E$+$01 & (9E$+$00,1E$+$01) & 26.64\\
57681.64 & $F160W$ & 1.21E$+$02 & (7E$+$00,5E$+$00) & 5.03E$+$01 & (5E$+$00,7E$+$00) & 3.59E$+$01 & (5E$+$00,7E$+$00) & 8.16E$+$00 & (6E$+$00,6E$+$00) & 25.76\\
57685.91 & $F625W$ & 5.58E$+$01 & (5E$+$00,2E$-$01) & 1.80E$+$01 & (2E$+$00,6E$-$01) & 5.64E$+$00 & (7E$-$01,6E$-$01) & 1.38E$+$00 & (5E$-$01,7E$-$01) & 25.42\\
57685.92 & $F814W$ & 1.15E$+$02 & (3E$+$00,0E$+$00) & 4.06E$+$01 & (1E$+$00,0E$+$00) & 1.29E$+$01 & (8E$-$01,4E$-$01) & 6.90E$+$00 & (7E$-$01,5E$-$01) & 24.99\\
57685.93 & $F475W$ & 8.44E$+$00 & (1E$+$00,0E$+$00) & 3.07E$+$00 & (5E$-$01,0E$+$00) & 7.50E$-$01 & (4E$-$01,0E$+$00) & $-$2.87E$-$01 & (4E$-$01,0E$+$00) & 25.58\\
57685.94 & $F390W$ & 5.67E$-$01 & (2E$-$01,0E$+$00) & 2.02E$-$01 & (2E$-$01,0E$+$00) & 3.54E$-$01 & (2E$-$01,0E$+$00) & $-$1.12E$-$01 & (2E$-$01,0E$+$00) & 25.24\\
57685.99 & $F110W$ & 4.15E$+$02 & (1E$+$01,1E$+$01) & 2.03E$+$02 & (9E$+$00,1E$+$01) & 1.26E$+$02 & (8E$+$00,1E$+$01) & 4.37E$+$01 & (9E$+$00,1E$+$01) & 26.64\\
57685.99 & $F160W$ & 1.21E$+$02 & (9E$+$00,0E$+$00) & 5.66E$+$01 & (6E$+$00,6E$+$00) & 4.67E$+$01 & (6E$+$00,6E$+$00) & 2.63E$+$00 & (7E$+$00,4E$+$00) & 25.76\\
57689.91 & $F625W$ & 4.09E$+$01 & (3E$+$00,6E$-$01) & 1.36E$+$01 & (1E$+$00,7E$-$01) & 4.27E$+$00 & (5E$-$01,7E$-$01) & 6.12E$-$01 & (4E$-$01,7E$-$01) & 25.42\\
57689.91 & $F814W$ & 9.39E$+$01 & (2E$+$00,4E$-$01) & 3.36E$+$01 & (1E$+$00,7E$-$01) & 9.43E$+$00 & (5E$-$01,8E$-$01) & 5.61E$+$00 & (5E$-$01,8E$-$01) & 24.99\\
57689.96 & $F110W$ & 5.20E$+$02 & (1E$+$01,1E$+$01) & 2.08E$+$02 & (9E$+$00,1E$+$01) & 1.05E$+$02 & (8E$+$00,2E$+$01) & 2.40E$+$01 & (9E$+$00,1E$+$01) & 26.64\\
57689.96 & $F160W$ & 1.90E$+$02 & (7E$+$00,5E$+$00) & 7.00E$+$01 & (5E$+$00,7E$+$00) & 4.06E$+$01 & (5E$+$00,7E$+$00) & $-$2.67E$+$00 & (6E$+$00,6E$+$00) & 25.76\\
57694.21 & $F625W$ & 3.44E$+$01 & (3E$+$00,7E$-$01) & 1.17E$+$01 & (1E$+$00,8E$-$01) & 3.83E$+$00 & (4E$-$01,8E$-$01) & 2.47E$-$01 & (2E$-$01,8E$-$01) & 25.42\\
57694.21 & $F814W$ & 8.70E$+$01 & (2E$+$00,6E$-$01) & 2.97E$+$01 & (8E$-$01,8E$-$01) & 9.43E$+$00 & (4E$-$01,8E$-$01) & 5.32E$+$00 & (4E$-$01,8E$-$01) & 24.99\\
57694.24 & $F110W$ & 5.97E$+$02 & (1E$+$01,1E$+$01) & 1.77E$+$02 & (8E$+$00,1E$+$01) & 9.54E$+$01 & (8E$+$00,2E$+$01) & 2.45E$+$01 & (9E$+$00,1E$+$01) & 26.64\\
57694.24 & $F160W$ & 2.34E$+$02 & (8E$+$00,2E$+$00) & 8.63E$+$01 & (6E$+$00,6E$+$00) & 4.13E$+$01 & (6E$+$00,6E$+$00) & 1.37E$+$01 & (7E$+$00,5E$+$00) & 25.76\\
57698.25 & $F625W$ & 2.92E$+$01 & (2E$+$00,7E$-$01) & 1.01E$+$01 & (9E$-$01,8E$-$01) & 3.49E$+$00 & (4E$-$01,8E$-$01) & 2.28E$-$01 & (3E$-$01,8E$-$01) & 25.42\\
57698.25 & $F814W$ & 7.15E$+$01 & (2E$+$00,6E$-$01) & 2.49E$+$01 & (7E$-$01,7E$-$01) & 7.29E$+$00 & (4E$-$01,8E$-$01) & 4.61E$+$00 & (4E$-$01,8E$-$01) & 24.99\\
57698.26 & $F110W$ & 4.60E$+$02 & (1E$+$01,1E$+$01) & 1.47E$+$02 & (8E$+$00,1E$+$01) & 8.85E$+$01 & (8E$+$00,2E$+$01) & 2.17E$+$01 & (9E$+$00,1E$+$01) & 26.64\\
57698.26 & $F160W$ & 2.04E$+$02 & (7E$+$00,5E$+$00) & 7.36E$+$01 & (5E$+$00,7E$+$00) & 4.45E$+$01 & (5E$+$00,7E$+$00) & 1.47E$+$01 & (6E$+$00,6E$+$00) & 25.76\\
57702.16 & $F625W$ & 1.74E$+$01 & (1E$+$00,8E$-$01) & 8.52E$+$00 & (8E$-$01,8E$-$01) & 2.90E$+$00 & (3E$-$01,8E$-$01) & 3.09E$-$01 & (2E$-$01,8E$-$01) & 25.42\\
57702.16 & $F814W$ & 6.03E$+$01 & (2E$+$00,7E$-$01) & 1.96E$+$01 & (6E$-$01,8E$-$01) & 6.81E$+$00 & (4E$-$01,8E$-$01) & 3.73E$+$00 & (4E$-$01,8E$-$01) & 24.99\\
57702.17 & $F110W$ & 3.24E$+$02 & (1E$+$01,1E$+$01) & 1.30E$+$02 & (8E$+$00,1E$+$01) & 8.54E$+$01 & (8E$+$00,2E$+$01) & 3.05E$+$01 & (9E$+$00,1E$+$01) & 26.64\\
57702.17 & $F160W$ & 1.75E$+$02 & (8E$+$00,2E$+$00) & 6.87E$+$01 & (6E$+$00,6E$+$00) & 3.72E$+$01 & (6E$+$00,6E$+$00) & 1.18E$+$01 & (7E$+$00,5E$+$00) & 25.76\\
57707.12 & $F625W$ & 1.87E$+$01 & (2E$+$00,7E$-$01) & 7.07E$+$00 & (7E$-$01,8E$-$01) & 3.13E$+$00 & (4E$-$01,8E$-$01) & $-$7.55E$-$02 & (3E$-$01,8E$-$01) & 25.42\\
57707.12 & $F814W$ & 4.97E$+$01 & (1E$+$00,7E$-$01) & 1.76E$+$01 & (6E$-$01,8E$-$01) & 5.74E$+$00 & (4E$-$01,8E$-$01) & 2.90E$+$00 & (4E$-$01,8E$-$01) & 24.99\\
57707.14 & $F110W$ & 2.89E$+$02 & (1E$+$01,1E$+$01) & 1.05E$+$02 & (8E$+$00,1E$+$01) & 7.37E$+$01 & (8E$+$00,2E$+$01) & 7.85E$+$00 & (9E$+$00,1E$+$01) & 26.64\\
57707.14 & $F160W$ & 1.33E$+$02 & (7E$+$00,4E$+$00) & 5.81E$+$01 & (5E$+$00,7E$+$00) & 3.78E$+$01 & (5E$+$00,7E$+$00) & 9.04E$+$00 & (6E$+$00,6E$+$00) & 25.76\\
57709.72 & $F625W$ & 2.15E$+$01 & (2E$+$00,7E$-$01) & 7.16E$+$00 & (7E$-$01,8E$-$01) & 2.74E$+$00 & (3E$-$01,8E$-$01) & $-$7.33E$-$02 & (2E$-$01,8E$-$01) & 25.42\\
57709.74 & $F814W$ & 4.72E$+$01 & (1E$+$00,7E$-$01) & 1.75E$+$01 & (6E$-$01,8E$-$01) & 5.32E$+$00 & (4E$-$01,8E$-$01) & 2.56E$+$00 & (4E$-$01,8E$-$01) & 24.99\\
57709.78 & $F110W$ & 1.94E$+$02 & (1E$+$01,1E$+$01) & 1.04E$+$02 & (8E$+$00,1E$+$01) & 7.79E$+$01 & (8E$+$00,2E$+$01) & 7.60E$+$00 & (9E$+$00,1E$+$01) & 26.64\\
57709.78 & $F160W$ & 1.19E$+$02 & (8E$+$00,2E$+$00) & 5.13E$+$01 & (6E$+$00,6E$+$00) & 3.57E$+$01 & (6E$+$00,6E$+$00) & 5.26E$+$00 & (7E$+$00,5E$+$00) & 25.76\\
57714.32 & $F625W$ & 2.02E$+$01 & (2E$+$00,7E$-$01) & 6.66E$+$00 & (6E$-$01,8E$-$01) & 2.84E$+$00 & (4E$-$01,8E$-$01) & 1.98E$-$01 & (3E$-$01,8E$-$01) & 25.42\\
57714.32 & $F814W$ & 4.19E$+$01 & (1E$+$00,7E$-$01) & 1.49E$+$01 & (5E$-$01,8E$-$01) & 4.98E$+$00 & (4E$-$01,8E$-$01) & 2.58E$+$00 & (4E$-$01,8E$-$01) & 24.99\\
\hline\hline
\end{tabular}

